Position-Normal Manifold for Efficient Glint Rendering on High-Resolution Normal Maps

Detailed microstructures on specular objects often exhibit intriguing glinty patterns under high-frequency lighting, which is challenging to render using a conventional normal-mapped BRDF. In this paper, we present a manifold-based formulation of the glint normal distribution functions (NDF) that precisely captures the surface normal distributions over queried footprints. The manifold-based formulation transfers the integration for the glint NDF construction to a problem of mesh intersections. Compared to previous works that rely on complex numerical approximations, our integral solution is exact and much simpler to compute, which also allows an easy adaptation of a mesh clustering hierarchy to accelerate the NDF evaluation of large footprints. Our performance and quality analysis shows that our NDF formulation achieves similar glinty appearance compared to the baselines but is an order of magnitude faster. Within this framework, we further present a novel derivation of analytical shadow-masking for normal-mapped diffuse surfaces -- a component that is often ignored in previous works.

==> equations/approximation.tex <==
\begin{equation}
\min_{\bm{\alpha},\bm{Q}}(P'(\bm{\omega})^2-P(\bm{\omega})^2)^2
\Rightarrow
\tfrac{1}{2}\bm{\omega}_{z}+\sqrt{\bm{\omega}_{\smash{z}}^{\smash{2}}+\bm{\omega}^{\smash{\top}}_{\smash{xy}}\bm{Q}^\top\text{diag}(\bm{\alpha^2})\bm{Q}\bm{\omega}_{\smash{xy}}}
%\tfrac{1}{4}\bm{\omega}^\top_{xy}\bm{\Omega}\bm{\omega}_{xy}
%=P(\bm{\omega})^2.
\end{equation}
